Zero-shot Retrieval: Augmenting Pre-trained Models with Search Engines

Large pre-trained models can dramatically reduce the amount of task-specific data required to solve a problem, but they often fail to capture domain-specific nuances out of the box. The Web likely contains the information necessary to excel on any specific application, but identifying the right data a priori is challenging. This paper shows how to leverage recent advances in NLP and multi-modal learning to augment a pre-trained model with search engine retrieval. We propose to retrieve useful data from the Web at test time based on test cases that the model is uncertain about. Different from existing retrieval-augmented approaches, we then update the model to address this underlying uncertainty. We demonstrate substantial improvements in zero-shot performance, e.g. a remarkable increase of 15 percentage points in accuracy on the Stanford Cars and Flowers datasets. We also present extensive experiments that explore the impact of noisy retrieval and different learning strategies.

==> intro-old1.tex <==

Current machine learning practice involves training a model using a fixed dataset that, once trained, remains unchanged throughout its life. Consequently, when encountering an instance with a novel category, there is no way for it to react adequately. That has given rise to the current approach of utilizing massive datasets to train large models with billions of parameters to memorize as much input and output space as possible \cite{chen2021emerging}. However, not only is this approach costly and time-consuming but there is also no guarantee that it helps the final task of interest. That is because we cannot possibly sample the whole distribution and having larger memory encourages the model to memorize biases and spurious features that could hinder the downstream task \cite{lee2019few}. In addition, in certain applications of machine learning such as visual question answering or visual dialogue, the model almost certainly encounters unseen inputs and relying solely on a fixed training set, even if memorized in a large model, is infeasible. All in all, it is impossible to a priori train an all-knowing model that is suitable for every future input.

Some machine learning approaches allow the model to access some form of external data beyond the training stage. However, that usually remains limited to a fixed repository. In addition, sorting and retrieving the correct piece of information in those repositories could be a challenge on its own, especially if they are large \cite{wang2020survey,xiong2021answering}.

On the other hand, humans rely on the internet as a virtually infinite source of timely information for their learning and improvement. This enables humans to undertake learning throughout their life by actively seeking a constantly evolving knowledge source, i.e. the internet. Encountering an unknown task/instance prompts an inquiry leading to an ever-improving understanding of the world. Thus, search engines—the gatekeepers of this vast knowledge source—have become increasingly essential and enormous investments have been made to improve and maintain them. As such, after more than two decades of investment and continuous development, they are at the stage that impressively recognize the intent behind the queries and retrieve relevant information very well. That begs the question: if humans rely ever-increasingly on search engines to improve, why are not the current machine learning methods utilizing this unique technology too?

To that end, we consider a paradigm-shifting approach to machine learning in which the learning algorithm can utilize a search engine such as Google to seek the information it needs at test time to improve its performance. More specifically, using a search engine and formulating an appropriate query in natural language, a learning algorithm could obtain the inductive biases needed for prediction in the absence of labeled data. Data collected from the search engines provide weak supervision for enhancing the model. Instead of using a fixed knowledge base, this approach enables us to retrieve real-time, up-to-date, relevant information from various modalities, including text, images and videos \cite{yang2020leveraging,miech2019howto100m}.

The success of this approach hinges on the ability of the learning algorithm to utilize natural language to ground the concepts as much as possible. With recent advances in language models such as OpenAI's GPT-3 \cite{brown2020language}, significant progress is made to enable machines to interact and process text. When combined with other modalities such as jointly learning image and text in OpenAI's CLIP \cite{radford2021learning} or Google's ALIGN \cite{radford2021learning}, or video and text in VideoBERT \cite{sun2019videobert}, visual models improve. Additionally, self-supervised learning and generative modeling have shown promise for learning from noisy labels. Utilizing these technologies enable us to take a leap forward that otherwise would not be possible.

\begin{figure} % {r}{0.8\linewidth}
\centering
\includegraphics[width=0.75\textwidth]{figs/search_model.pdf}
\caption{The proposed framework: at inference time, given an input, the model determines whether it is uncertain, at which case additional data is retrieved, and the model is updated. The theoretical model and how it is trained are detailed in Task 1. In Task 2, it is used at inference time to generate a query and retrieve data.}
\label{fig:model}
% \vspace{-3mm}
\end{figure}


Our proposal presents a timely and highly impact approach to enhancing current learning paradigms. We believe this approach takes steps towards the next generation of learning algorithms for vision and language tasks by improving the test time performance using a human-like approach of employing search engines for producing the desired output.

\textbf{Questions:}
\begin{itemize}[leftmargin=*,topsep=1pt,itemsep=2ex,parsep=-1ex]
    \item how to quantify uncertainty when using such pre-trained models?
    \item Do they remember all they were trained on?
    \item Can we use instances from internet and adapt the models using weakly supervised signals?
    \item How effective is a pre-trained model such as CLIP in choosing the best search query? what could be a strategy to improve them?
\end{itemize}

The contributions of this paper are:
\begin{enumerate}[leftmargin=*,topsep=1pt,itemsep=2ex,parsep=-1ex]
    \item New approach to learning
    \item 
    \item Improved performance to zero-shot classification 
\end{enumerate}


==> intro-old2.tex <==


%\todo[inline]{
%Contribution: We propose constructing a dataset that provides robustness to current methods to novel views. The dataset is constructed in an online and novel fashion by retrieving images from search engines for the uncertain classes. 

%Problem: Current methods adapt to novel views using different techniques (). However, no one has tried to construct an online dataset for the difficult/uncertain classes for the method. 

%Evaluation: We evaluate our retrieval technique on multiple methods (CLIP, Tip-Adapter, more?) and datasets (Oxford cars, Food, Pets, ImageNet 1000k.)}

%task
%State-of-the-art
%flaw in the state of the art
%our solution
%results/evaluation proving that works.
\DT{This first paragraph has little to do with this paper (it could be the start of pretty much any ML paper written today. You should compress all this info to much less, maybe 2 sentences, and say something much more specific to what you want to achieve. What is your ultimate goal? Make it unambiguous from the start, then you can expand in the following paragraphs as currently done. Example: current ML models, despite advancements of large pretrained models, are limited because they are anchored to one particular snapshot of data. We want to create models that reflect the changing nature of the world, that can incorporate new knowledge on-the-fly, and generalize to new concepts.}
Current machine learning methodologies in computer vision and natural language processing tasks predominantly hinge on the utilization of large pre-trained models, subsequently fine-tuned for specific tasks. These models have predominantly emerged from the realm of self-supervised and unsupervised learning objectives. They are typically tailored for single modalities, such as images, exemplified by well-known instances like SimCLR \cite{simclr}, MoCo \cite{moco}, and DINO \cite{dino}, or text-based models, exemplified by pioneering models like GPT \cite{brown2020language} and LLama \cite{llama}. Additionally, we observe the emergence of multimodal models such as CLIP \cite{radford2021learning}, Flamingo \cite{flamingo}, ALIGN \cite{radford2021learning}, and ImageBind \cite{girdhar2023imagebind} that seamlessly combine text and images.
These pre-trained models exhibit a remarkable trajectory of growth, characterized by increasing size, precision, and proficiency, particularly in zero-shot learning scenarios. As time unfolds, we anticipate these models will continue their trajectory of enhancement, further solidifying their role as formidable zero-shot learners in the machine-learning landscape. 

% However, as these models improve as zero-shot learners, especially for common concepts, the need for highly curated datasets diminishes.
Pre-trained models, whether used as zero-shot learners or fine-tuned on a predefined downstream task dataset, exhibit limitations in handling unseen instances. Although the adoption of massive models with billions of parameters has been explored to mitigate these limitations \cite{chen2021emerging}, this approach is resource-intensive, time-consuming, and lacks guaranteed performance improvements in the target downstream task. Furthermore, the challenges of exhaustively sampling the entire data distribution, the risk of larger models memorizing biases and spurious features \cite{lee2019few}, and the potential distribution shift for concepts unaddressed by fixed models must be considered.

One approach to remedy this issue has been retrieval-augmented inference \cite{realm,seeker_retrieval,rapre} aiming to retrieve instances to help with generalisation. These approaches typically require the additional dataset to be available and learn to find similar representations to retrieve in addition to the given task. However, retrieving the pertinent information presents its own set of challenges besides computational cost~\cite{wang2020survey,xiong2021answering}.

Over the past two decades, substantial investments and continuous advancements have impressively enabled search engines to decipher user intent and retrieve pertinent information. Search engines have revolutionized human learning, enabling the retrieval of a wealth of diverse yet pertinent information through concise natural language queries. With just a few words, individuals can tap into a vast reservoir of knowledge, significantly enhancing their understanding and access to valuable information. That begs the question: if humans rely ever-increasingly on search engines to improve, why are not the current machine learning methods utilizing this unique technology, too? In particular, these large pre-trained models trained on internet-scale data presumably observed samples from  major concepts of general interest.

% Humans rely on the internet as a virtually infinite source of timely information for their learning and improvement. This enables humans to undertake learning throughout their life by actively seeking a constantly evolving knowledge source, i.e. the internet. Encountering an unknown task/instance prompts an inquiry leading to an ever-improving understanding of the world. Thus, search engines—the gatekeepers of this vast knowledge source—have become increasingly essential and enormous investments have been made to improve and maintain them. As such, after more than two decades of investment and continuous development, they are at the stage that impressively recognize the intent behind the queries and retrieve relevant information very well. 


This question is particularly timely since, with the remarkable success of large language models (LLMs), there is an increasing interest in using natural language to ground other modalities. 
In response, we explore the synergy between pre-trained models, which capture rich concept priors, and search engines, which have evolved to retrieve diverse and representative information based on textual queries efficiently. We propose a methodology where a few examples from search engine results compose the support set, enabling fine-tuning of the pre-trained model for improved predictions. In particular, since fine-tuning typically involves only a minimal update to model parameters \cite{lora}, we learn a small model for the task from this retrieved support set. 

In the future, we envision a dynamic approach where pre-trained models have the capability to access the internet to acquire new knowledge as they encounter novel concepts for prediction. This stands in contrast to traditional task-specific static models, which are expected to perform adequately even in the presence of previously unseen instances, a challenge that current out-of-distribution generalization research is striving to address. 

Our approach distinguishes itself from traditional active learning methods \citep{settles2010active}, where the primary objective is to judiciously request labels for specific data points within a fixed dataset. In sharp contrast, our approach, analogous to Internet Explorer, continuously expands its dataset without any reliance on pre-existing labels, even from the target dataset. Additionally, previous research efforts have explored ways to harness the internet as an auxiliary data source. For instance, NELL~\cite{carlson2010toward} introduced a method for systematically scraping web content to acquire new concepts and relationships, which are periodically refined with human supervision. NEIL~\cite{chen2013neil} extended NELL's approach to incorporate visual data and relationships. These methods are characterized as semi-supervised and aimed at accumulating broad ``common-sense" knowledge from the web. In contrast, our approach employs an actively improving ``directed" search strategy to excel on target data, all while operating in a fully self-supervised manner. Recent research~\cite{jiang2017deep}, while sharing a similar context, conducts searches within a static dataset rather than venturing onto the internet.

% As such, we believe there is a need to investigate the potential of using a combination of pre-trained models--which supposedly learn the best features to represent various concepts--with search engines--which in the past twenty years matured to be highly capable of finding diverse and representative information pieces given a query text. A small number of examples retrieved from the search engines provide the support set with which the pre-trained model can be updated for best predictions. In addition, it is shown that a small number of parameters are typically updated during finetuning. 

% and incorporate their priors as inductive biases in other applications. 

\DT{The intro is too bold with too-few references to existing areas of the literature. The ideas are good but they are brought in out of the blue: it is much safer to ground the discussion in past work that is directly relevant: active learning, webly-supervised learning, and all the work on learning to interact with search engines (learning to retrieve, query reformulation, query expansion).}
To that end, we consider a novel approach to machine learning in which the learning algorithm can utilize a search engine such as Google to seek the information it needs at test time to improve its performance. More specifically, using a search engine and formulating an appropriate query in natural language, a learning algorithm could obtain the inductive biases needed for prediction in the absence of labelled data. Data collected from the search engines provide weak supervision for enhancing the model. Instead of using a fixed knowledge base, this approach enables us to retrieve real-time, up-to-date, relevant information from various modalities, including text, images and videos \cite{yang2020leveraging,miech2019howto100m}.
The success of this approach hinges on the ability of the learning algorithm to utilize natural language to ground the concepts as much as possible. 

In other words, the descriptiveness of the labels provided with each downstream dataset directly correlates with the usefulness of the retrieved data. An implication of this is that a better fine-tuned accuracy is expected as the specificity of the labels increases. For example, in the case of labels that describe a manufactured item like a car, the overall shape and looks of a make and model will not vary between a curated dataset (that focuses on a certain narrow part of the distribution of images from that car) and a dataset that is made up of images retrieved from a search engine. However, in the case of food images, the recipes and final looks of a dish can vary significantly because of the subjective elements involved in making a certain dish. This change can potentially result in distribution shifts between the images from the curated dataset and retrieved images.

We investigate this problem in the context of visual classification using a pre-trained model such as CLIP.
Note that while we focus our attention on a pre-trained CLIP, our approach is generic and can be applied to models trained on a downstream task.

Our proposal presents a timely, highly impactful approach to enhancing current learning paradigms. We call our approach \emph{proactive learning} since the model proactively seeks additional information for effective prediction.
We believe this approach takes steps towards the next generation of learning algorithms for vision and language tasks by improving the test time performance using a human-like approach of employing search engines for producing the desired output. 
In the process of developing this approach, we investigate the extent in which CLIP is uncertain about different concepts and how it benefits from extra data. In addition, we investigate the best approach to update or fine-tune CLIP with this small retrieved dataset.

\DT{At this point it is still not clear why this approach is not just a variant of active learning (which is the first thing that will come to mind to the reader). Rebranding an existing concept with a new name is very bad, so we must make it very clear that it's not the case. Why also isn't this just another retrieval-augmented model (which there have been quite a few recently)?}

The contributions of this paper are\hl{to revise}:
\begin{itemize}[leftmargin=*,topsep=1pt,itemsep=2ex,parsep=-1ex]
    \item We propose a novel learning paradigm in which a search engine supplements a pre-trained model for prediction
    \item We perform extensive analysis  to understand better the best query, the effectiveness of identifying uncertain instances, the quality of the retrieved images, and the concepts that can best benefit from such an approach
    \item Our experiments show in predictions on classes such as CAR, we observe more than 15\% improvement in classification accuracy.
\end{itemize}


==> results/cars_confidence_boxplot.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\textwidth]{figs/cars_confidence_boxplot.png}
    \caption{Cars}
    \label{fig:cars_confidence_boxplot}
\end{figure}

==> results/classes_that_improve.tex <==
% \todo[inline]{analysis on the classes that improve.}

==> results/expected_calibration_error.tex <==
\begin{table}[h]
% \setlength{\tabcolsep}{2.pt}
\caption{Expected calibration error}
\label{tab:ece}
\centering
\begin{tabular}{@{}lcccc@{}}
\shortstack{Dataset}  & \shortstack{ECE before} & \shortstack{ECE after} \\
\toprule
StanfordCars & 0.0410 & 0.0283 \\
Flowers102 & 0.0397 & 0.0565 \\
OxfordIIITPet & 0.0367 & 0.0374 \\
Food101 & 0.0310 & 0.0516 \\
\end{tabular}
\end{table}

==> results/pets_confidence_boxplot.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\textwidth]{figs/pets_confidence_boxplot.png}
    \caption{Pets}
    \label{fig:pets_confidence_boxplot}
\end{figure}

==> results/search_imgs.tex <==
% \begin{table}[t]
\begin{wraptable}[]{}{}
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{clllll}
\toprule
       & \multicolumn{1}{c}{Flowers} & \multicolumn{1}{c}{Pets} & \multicolumn{1}{c}{Cars} & \multicolumn{1}{c}{Food} \\ \midrule%& \multicolumn{1}{c}{ImageNet} \\\midrule%(lr){5-9}
 \textit{ZeroShot CLIP-B-16}& 71.15                       & 89.04                    & 64.71                    & 88.73  \\ %& 68.33                        \\ 
 \textit{Search Image using LAION-5B}& 61.86 \downr{-9.29}         & 80.84 \downr{-8.20}      & 56.60 \downr{-8.10}      & 88.35 \downr{-0.38}      &                              \\
\bottomrule
\end{tabular}%
}
\caption{Accuracy results by training our method with searching images by certain images using LAION-5B}
\label{tab:image_based_retrieved}
% \vspace{-2em}
% \end{table}
\end{wraptable}

==> results/shannon_entropy.tex <==
\begin{table}
\centering
\caption{Ablation on the threshold for Shannon entropy}
\label{tab:threhold_ablation}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}lccccc@{}}
\shortstack{Dataset } & \shortstack{CLIP} & \shortstack{0.3} & \shortstack{0.5} & \shortstack{0.7} & \shortstack{0.9} \\
\toprule
StanfordCars-Top1 & 64.10\% & 64.17\% & 77.43\% & 81.16\% & 81.83\% \\
StanfordCars-Top3 & 87.98\% & 87.45\% & 90.51\% & 95.08\% & 95.45\% \\
Flowers102-Top1 & 66.07\% & - & 78.03\% & 79.89\% & 79.88\% \\
Flowers102-Top3 & 79.55\% & - & 84.02\% & 86.75\% & 86.70\% \\
OxfordIIITPet-Top1 & 85.77\% & 85.79\% & 87.75\% & 87.24\% & 87.85\% \\
OxfordIIITPet-Top3 & 96.23\% & 95.12\% & 95.68\% & 94.75\% & 95.00\% \\
Food101-Top1 & 84.25\% & 84.16\% & 84.43\% & 84.34\% & 84.34\% \\
Food101-Top3 & 95.15\% & 93.35\% & 93.80\% & 93.63\% & 93.63\% \\
\end{tabular}
\end{table}

==> results_vqa.tex <==

\section{Results on the Learning using external sources}
\label{sec:results}

\par{\textbf{Problem Setup and the Baseline}}

In this report, we first reproduced the baseline CLIP-ViL \cite{clip-vqa} for the VQA2.0~\cite{antol2015vqa} on the minival set, which consists of a test set with publicly available ground truth. For the propose minival set, the pre-trained model CLIP-ViL achieved $71.00$ \% of accuracy. We then further fine-tune the model for the downstream task VQA2.0, which achieved an overall accuracy of $73.93$ \%. We report the model performance on Table ~\ref{tab:overal}.  %The paper states an accuracy of $76.7$\% on test-std ( test set where ground truth is not publicly available).

This accuracy is also obtainable by submitting the generated predictions from the VQA fine-tuned CLIP-ViL model to the test server. For the experiments we performed, we used the CLIP ViL VQA fine-tuned checkpoint as the baseline.

The questions from the minival set which the fine-tuned baseline answered incorrectly are referred to as the minival-incorrect set for the experiments. We believe the main benefit could be brought to improving the incorrectly predicted answers.

%-------------------------------------------------
%-------------------------------------------------
\begin{table*}[t]
    \centering
    \begin{tabular}{rcc}
\toprule
        \textbf{Model} & 
\textbf{Incorrect set Acc.} & 
\textbf{Incorrect Filtered-set Acc.} \\
\midrule
CLIP-ViL-VQA  \cite{clip-vqa} &
0 &
0 \\
CLIP-ViL-VQA + keywords &
12.28 & 
\textbf{14.56} \\
CLIP-ViL-VQA + image caption &
11.43 &
\textbf{11.69} \\
\bottomrule
    \end{tabular}
    \caption{Minival-incorrect set experiments}
    \label{tab:incorrectset}
\end{table*}

%-------------------------------------------------
%-------------------------------------------------
\begin{table}
    \centering
    \begin{tabular}{lc}
    \toprule
Model & Acc. \\
\midrule
CLIP-ViL \cite{clip-vqa} &
71.00 \\
CLIP-ViL-VQA &  \textbf{73.93} \\
CLIP-ViL-VQA + keywords & 71.57 \\
CLIP-ViL-VQA + image caption & 72.40 \\
\bottomrule
    \end{tabular}
    \caption{When all the examples are used to be fine-tuned}
    \label{tab:overal}
\end{table}

%JS: looks like its not complete from here on.
\par{\textbf{Fine-tuning on unseen data}}


We perform additional fine-tuning into two distinct experiments. First, we further optimize the CLIP-ViL model with a set of keywords, following the proposed learning by search approach. In this step, we utilized keywords decomposed from hard questions as queries for Google Image search, then the retrieved images were leveraged on the optimization of the model. To determine whether there is a benefit in fine-tuning CLIP on unseen data, we selected a few keywords relating to the concept of a ‘man cave’ which the model has not been trained on. The dataset for fine-tuning consisted of data obtained from web crawled images where the search term was one of the following: {‘mancave’, ‘mancave bar’, ‘mom cave’, ‘man cave’, man caves’, ‘man cave bar’, ‘man cave couch’, ‘mantuary’, ‘woman cave’}. We used this as a simple baseline to ensure the validity of the hypothesis. We name name this approach \textbf{CLIP-ViL-VQA + keywords}.

The second approach consists of utilizing image captioning for querying the images from Google Image Search. We define the captioning of images as follows:
(1) using the search term as the only caption, (2) simulating some generic sentences that included the search term, and (3) using the google image title as the caption. 
The retrieved images are utilized to fine-tune the CLIP-VQA model, which we denote as \textbf{CLIP-ViL-VQA + image captions}. For this experiment, we also report the models' performance on Table~\ref{tab:overal}.

Finally, we select a subset of incorrect labelled samples by the CLIP-ViL-VQA model from the minival VQA2.0. In this experiment we aim to evaluate whether the fine-tuning step leveraging the man cave images have a positive impact on the CLIP-ViL-VQA.
%of the validation dataset These datasets were then evaluated on a selection of unseen man cave images and custom questions. 
We observed that for this small subset, we could achieve 3\% improvement compared to the baseline highlighting the validity of the hypothesis. 

\subsection{Incorrect set experiments}

\par{\textbf{Fine-tuning on unseen data}}

We applied the EASE metric on the ground truth of the minival-incorrect set, which allowed us to create a filtered subset of data to use for fine-tuning. For this step, we consider 
%  based on the following criteria on the question-image tuples. We c
(1) 0.2 $<$ EASE $<$ 0.7 for the triplets, which are sufficiently reasonable to answer, (2) questions categorized as ‘what’ since that is more likely be related to inquiring concepts and excluding ‘how many, ‘what time’ that potentially don't benefit from our approach.

Noun-phrase keywords were extracted from the questions in the minival-incorrect set filtered based on the above conditions. These noun phrases were used to generate a google crawled dataset. That is, we used google image search using that query word (as shown in Figure~\ref{fig:model}).

We then created captions for the images in two different ways (1) using the search term as the only caption, and (2) using the google image title caption. We observed that keywords for the google crawl relate to many different concepts, which poses a challenge to simulate questions that relate to the data in a generic way. For this, we explored ConceptNet~\cite{speer2017conceptnet}. We further present our findings using ConceptNet in the next section.

For the two models that were fine-tuned, a summary of the results is provided in Table~\ref{tab:mancave}:
% \begin{table*}[]
%     \centering
%     \includegraphics[width=\textwidth]{latex/img/bike_ft_clip.pdf}
%     \caption{An example of using the google search on Bike}
%     \label{tab:my_label}
% \end{table*}
\begin{table*}[]
    \centering
    \hspace{-35mm}\vspace{-30mm}
    \includegraphics[width=1.2\textwidth,height=24.5cm]{latex/img/clip-vil-mancave-211028 - mancave-211028-Ehsans-dataset.pdf}
    \caption{\vspace{-10mm}Examples of improvements on the mancave retrieval}
    \label{tab:mancave}
\end{table*}
From table \ref{tab:overal}, there is an overall decrease in accuracy after fine-tuning compared to the VQA fine-tuned baseline by 1.53 - 2.36 %. A summary of predictions from the fine-tuned models on the minival set is available here: https://docs.google.com/spreadsheets/d/1BuETxd0Ond5HCaN9aie4KXTwb0EWtiEQUHrJKdClihE/edit?usp=sharing

We are still looking into which questions may benefit most from fine-tuning based on a number of metrics (EASE applied to the predicted data at different thresholds).

